Query-adaptive Recurrent Tokenization

Visual information worth extracting from an image and the token budget it warrants depend on the text query. Yet modern vision and vision-language models largely encode images independently of the query and allocate a fixed visual token budget to every input. We introduce the Query-Adaptive Recurrent Tokenizer (QART), a backbone-agnostic module that makes visual representations both query-steerable and budget-adaptive. QART steers the visual representation toward query-relevant evidence while adapting its token budget to the amount of information required. Its key principle is simple. Additional tokens are allocated until the visual features relevant to the query are represented with sufficient fidelity. Starting from frozen encoder features, QART recurrently constructs a compact representation and uses reconstruction quality over the query-relevant visual support to control token allocation. On Visual7W and VQAv2, QART achieves 81.96% and 76.37% accuracy using only about 29 visual tokens, reducing token counts by 20-25x relative to dense VLM inputs. It further reaches 92.0% P@1 on CORE and 36.3% PR-AUC on PODS, outperforming SteerViT on PODS by 8.4%. Together, these results show that visual representations need not be fixed in either content or capacity and can instead adapt to what each query requires.

==> figures/multipanel_figure_snippets.tex <==

% Requires:
% \usepackage{graphicx}
% \usepackage{subcaption}

% ------------------------------------------------------------------
% Figure 1: Representation quality and query dependence
% ------------------------------------------------------------------
\begin{figure*}[t]
    \centering
    \begin{subfigure}[t]{0.49\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/panel_core.pdf}
        \caption{CORE. QART substantially redirects the frozen SigLIP2 representation toward queried content.}
        \label{fig:rep_core}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.49\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/panel_genecis.pdf}
        \caption{GeneCIS. Query-conditioned representation learning transfers to natural images without task-specific tuning.}
        \label{fig:rep_genecis}
    \end{subfigure}

    \vspace{0.5em}

    \begin{subfigure}[t]{0.49\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/panel_winoground.pdf}
        \caption{Winoground. Removing query-specific conditioning substantially degrades Image and Group accuracy.}
        \label{fig:rep_winoground}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.49\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/panel_pods.pdf}
        \caption{PODS. Coarse query conditioning preserves fine-grained instance identity.}
        \label{fig:rep_pods}
    \end{subfigure}

    \caption{
        \textbf{QART changes what the visual representation encodes while preserving downstream information.}
        (a) Query conditioning strongly improves retrieval over fixed SigLIP2 representations on CORE.
        (b) The same representation transfers zero-shot to natural scenes on GeneCIS.
        (c) On Winoground, replacing the sample-specific query with a fixed query causes a large drop, showing that the representation is genuinely query-dependent.
        (d) On PODS, QART retains instance-level information even when conditioned only on a coarse supercategory prompt.
    }
    \label{fig:representation_results}
\end{figure*}


% ------------------------------------------------------------------
% Figure 2: Compactness, downstream utility, and efficiency
% ------------------------------------------------------------------
\begin{figure*}[t]
    \centering
    \begin{subfigure}[t]{0.49\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/panel_vqav2_tradeoff.pdf}
        \caption{VQAv2 accuracy versus visual-token budget.}
        \label{fig:eff_vqav2}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.49\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/panel_vqav2_budget.pdf}
        \caption{Average QART token budget across VQAv2 question types.}
        \label{fig:eff_budget}
    \end{subfigure}

    \vspace{0.5em}

    \begin{subfigure}[t]{0.49\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/panel_throughput.pdf}
        \caption{End-to-end VLM throughput as batch size increases.}
        \label{fig:eff_throughput}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.49\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/panel_speedup.pdf}
        \caption{End-to-end and language-model prefill speed-up over LLaVA-1.5-7B.}
        \label{fig:eff_speedup}
    \end{subfigure}

    \caption{
        \textbf{QART preserves downstream utility with a compact adaptive visual sequence and translates this compactness into inference gains.}
        (a) QART reaches 77.4\% VQAv2 accuracy with 29.4 visual slots on average, remaining close to the full 576-token LLaVA-1.5-7B model and above published methods at a comparable 32-token budget.
        (b) The allocated budget varies with question type, with counting receiving the largest average capacity.
        (c-d) The shorter visual sequence increasingly benefits batched inference, reaching 1.53$\times$ end-to-end and 2.54$\times$ prefill speed-up at batch size eight.
    }
    \label{fig:efficiency_results}
\end{figure*}


==> sections/acknowledgments.tex <==
\subsubsection*{Acknowledgments}


==> sections/author_contributions.tex <==
\subsubsection*{Author Contributions}


==> sections/preliminaries.tex <==
\section{Preliminaries and Problem Setup}
\label{sec:preliminaries}



